PeP: a Point enhanced Painting method for unified point cloud tasks

Point encoder is of vital importance for point cloud recognition. As the very beginning step of whole model pipeline, adding features from diverse sources and providing stronger feature encoding mechanism would provide better input for downstream modules. In our work, we proposed a novel PeP module to tackle above issue. PeP contains two main parts, a refined point painting method and a LM-based point encoder. Experiments results on the nuScenes and KITTI datasets validate the superior performance of our PeP. The advantages leads to strong performance on both semantic segmentation and object detection, in both lidar and multi-modal settings. Notably, our PeP module is model agnostic and plug-and-play. Our code will be publicly available soon.

==> exp.tex <==
\begin{figure*}[htbp]
\centering     

\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/32.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/34.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/58.jpg}}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``stop vehicle next to the man with a wheelchair."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``bob is waiting in the car on the left side of the road. i need to pick him up. make a you-turn when safely able to do so."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``that is my wife. stop next to her."
\end{minipage}

\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/82.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/103.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/119.jpg}}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``watch out for that guy, i think he might try to cross the street. better slow down."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``take a left turn after that silver car parked on the left."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``park just passed where that dog is."
\end{minipage}

\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/198.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/229.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/2379.jpg}}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``par in front of that old truck on the other side of the road."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``pull up next to that officer standing more on the road than the other one. i want to talk to him."
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``let the car on the left overtake you."
\end{minipage}

\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/2366.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/251.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
    \vspace{3pt}
    \centerline{\includegraphics[width=\textwidth]{exp_fig/101.jpg}}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``i see my friend mark. stop here for a moment"
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``pull up next to the guy wearing the safty vest so i can talk to him"
\end{minipage}
\begin{minipage}{0.3\linewidth}
\vspace{3pt}
    ``park behind the car infront of the mail truck"
\end{minipage}


\caption{\textbf{Visualization results on Talk2Car.} The green bounding box in the image corresponds to the ground truth, while the red bounding box represents the output generated by our model. The instruction corresponding to the image is provided below.}
\label{fig:qualitative}
\end{figure*}
